Over-parameterized Adversarial Training: An Analysis Overcoming the Curse of Dimensionality

Adversarial training is a popular method to give neural nets robustness against adversarial perturbations. In practice adversarial training leads to low robust training loss. However, a rigorous explanation for why this happens under natural conditions is still missing. Recently a convergence theory for standard (non-adversarial) supervised training was developed by various groups for {\em very overparametrized} nets. It is unclear how to extend these results to adversarial training because of the min-max objective. Recently, a first step towards this direction was made by Gao et al. using tools from online learning, but they require the width of the net to be \emph{exponential} in input dimension $d$, and with an unnatural activation function. Our work proves convergence to low robust training loss for \emph{polynomial} width instead of exponential, under natural assumptions and with the ReLU activation. Key element of our proof is showing that ReLU networks near initialization can approximate the step function, which may be of independent interest.

==> analysis.tex <==

\section{Convergence Analysis}


\subsection{Overview}
We first consider the dynamics of the continuous time domain. Denote $y = \sbr{y_1,\cdots,y_n}^\top \in \RR^n$, $f(t) = \sbr{ f_1(t),\cdots, f_n(t) }^\top \in \RR^n$, and $f_i(t) = f_{W(t),a}(x_i(t))$ for all $i \in [n]$. For each $r$, let $w_{r:}$ denote the $r$-th row of matrix $W$.

Consider the ordinary differential equation (ODE)
\begin{align*}
\frac{d~w_{r:}(t)}{d~t} = & ~ - \sum_{i=1}^n \frac{\partial \Phi ( W(t),a(t),x_i(t)) }{\partial ~w_{r:}(t)},\\
\frac{d~x_i(t)}{d~t} = & ~ - \frac{\partial \Phi (W(t),a(t),x_i(t)) }{\partial ~x_i(t)}, \\
\frac{d~a(t)}{d~t} = & ~ - \sum_{i=1}^n \frac{\partial \Phi ( W(t),a(t),x_i(t)) }{\partial ~a(t)}.
\end{align*}

For convenience, we consider $a$ to be fixed for now. Then
\begin{align*}
\frac{d~f_i(t)}{d~t} &= \left\langle \frac{\partial f ( W(t), a, x_i(t) ) }{\partial x_i(t)}, \frac{d~x_i(t)}{d~t} \right\rangle + \sum_{r=1}^m \left\langle \frac{\partial f ( W(t), a, x_i(t) ) }{\partial w_{r:}(t)}, \frac{d~w_{r:}(t)}{d~t} \right\rangle \\
&= ( y_j - f_j ) \left\langle \frac{\partial f ( W(t), a, x_i(t) ) }{\partial x_i(t)}, \frac{\partial f ( W(t), a, x_i(t) ) }{\partial x_i(t)} \right\rangle \\
&\hspace{0.5in}+ \sum_{j=1}^n ( y_j - f_j ) \sum_{r=1}^m \left\langle \frac{\partial f ( W(t), a, x_i(t) ) }{\partial w_{r:}(t)}, \frac{\partial f ( W(t), a, x_j(t) ) }{\partial w_{r:}(t)} \right\rangle \\
&= ( y_j - f_j ) H^{x}_{i}(t) + \sum_{j=1}^n ( y_j - f_j ) H^{w}_{ij}(t),
\end{align*}
where 
\begin{align*}
H^{w}_{i,j}(t) &= ~ \frac{1}{m} x_i^\top(t) x_j(t) \sum_{r=1}^{m}  \mathds{1}_{ w_{r:}^\top(t) x_i(t) \geq 0, w_{r:}^\top(t) x_j(t) \geq 0 },~\\
H^{x}_{i,i}(t) &= ~ \frac{1}{m} \sum_{r=1}^m ( \sum_{k=1}^d w_{rk} )^2 \mathds{1}_{w_{r:}^\top(t) x_i(t) \geq 0},~\text{and}~H^{x}_{i,j}(t) = 0~\text{for}~i \neq j.
\end{align*}
Then we have
\begin{align*}
\frac{d~f(t)}{d~t} = ( H^{w}(t) + H^{x}(t) ) ( y - f ).
\end{align*}

To show the convergence, we need to show that $H^{w}(t) + H^{x}(t)$ is PSD, i.e., $\lambda_{\min} ( H^{w}(t) + H^{x}(t) ) \geq 0$. Since $H^{x}(t)$ is diagonal and has non-negative entries, $H^{x}(t)$ is PSD. Then a weaker result is to show that $H^{w}(t)$ is PSD rather than $H^{w}(t) + H^{x}(t)$ directly.

Steps needed to show the convergence/divergence of the adversarial training.

\textbf{Step 1: } Show that $\lambda_{\min} ( H(0) ) \geq \frac{3 \lambda_0}{4}$ for some constant $\lambda_0 > 0$. In \cite{dzps19}, this is done by showing that $\|H(0) - H^{\infty} \|_2 \leq \frac{\lambda_0}{4}$ given $\lambda_{\min} ( H^{\infty} ) = \lambda_0$, where 
\begin{align*}
H_{i,j}^{\infty} = & ~ \E_{w \sim \N(0,I)} \left[ x_i^\top x_j \mathds{1}_{ w^\top x_i \geq 0, w^\top x_j \geq 0 } \right],
\end{align*}
and
\begin{align*}
H_{i,j}(0) = & ~ \frac{1}{m} x_i^\top(0) x_j(0) \sum_{r=1}^{m}  \mathds{1}_{ w_{r:}^\top(0) x_i(0) \geq 0, w_{r:}^\top(0) x_j(0) \geq 0 },
\end{align*}
I think $x_i$ in $H^{\infty}$ is $x_i(0)$, right? \Zhao{This is also confusing to me}

\textbf{Step 2: } Show that $\lambda_{\min} ( H(t) ) \geq \frac{\lambda_0}{2}$ for all $t>0$, where
\begin{align*}
H_{i,j}(t) = ~ \frac{1}{m} x_i^\top(t) x_j(t) \sum_{r=1}^{m}  \mathds{1}_{ w_{r:}^\top(t) x_i(t) \geq 0, w_{r:}^\top(t) x_j(t) \geq 0 },
\end{align*}
$x_i(t)$ and $w_{r:}(t)$ are obtained from the adversarial training for all $r \in [m]$ and $i \in [n]$. In \cite{dzps19}, this is done by showing that $\|H(0) - H(t) \|_2 \leq \frac{\lambda_0}{4}$ given $\|w_{r:}(t) - w_{r:}(0) \|_2$ is small, where $x_i$'s are fixed in $H(t)$. We can assume that both $\|w_{r:}(t) - w_{r:}(0) \|_2$ and $\|x_i(t) - x_t(0) \|_2$ are small, but note that in each iteration $t$, we have different $x_i(t)$. It seems in each iteration, we need to generate one data for each $x_i$ so that $H(t)$ and $H(0)$ have the same size $n \times n$. What should we do if the number of generated samples $n(t) \neq n$?

\textbf{Step 3: } Suppose $n(t) = n$, show that $\|y - f(t)\|_2^2 \leq \exp ( - \lambda_0 t ) \|y - f(0)\|_2^2$. 


\textbf{Step 4: } Calculate the gradient on $x$ with and without adversarial training. In specific, let $\Phi ( \hat{W},X )$ be the loss using the regular gradient descent (as in \cite{dzps19}) and $\Phi( \tilde{W},X )$ be the loss using the adversarial training. Then we compute
\begin{align*}
\nbr{ \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} }_2
~~~\text{and}~~~~
\nbr{ \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} }_2.
\end{align*}
If adversarial training works, then $\| \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} \|_2 > \| \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} \|_2$. Otherwise, they are of the same order.



We show
\begin{align*}
  (1-1/t)^t \| \wh{W}^t \|_2 \leq \| \wt{W}^t  - \wh{W}^t \|_2 \leq (1+1/t)^t \| \wh{W}^t \|_2
\end{align*}
Eventually, RNN proved somthing like this
\begin{align*}
  \frac{1}{t} \| \wh{W}^t \|_2 \leq \| \wt{W}^t  - \wh{W}^t \|_2 \leq t^2 \| \wh{W}^t \|_2
\end{align*}

\newpage
\subsection{Technical details}

We define the update of weights
\begin{definition}
Let $\wh{W}^t$ denote the classical training in iteration $t$, let $\wt{W}^t$ denote the weight matrix generated by adversarial training in iteration $t$. We $\wh{W}^t$ and $\wt{W}^t$ as follows:
\begin{align*}
    \wh{W}^{t} = & ~ \wh{W}^{t-1} - \eta \cdot \sum_{x_i \in D} \frac{ \partial \Phi(W,x_i) }{ \partial W } \Big|_{W = \wh{W}^{t-1}} \\
    \wt{W}^{t} = & ~ \wt{W}^{t-1} - \eta \cdot \sum_{ x_i \in D^t } \frac{ \partial \Phi(W,x_i) }{ \partial W } \Big|_{ W = \wt{W}^{t-1} } \\
    = & ~ \wt{W}^{t-1} - \eta \cdot \sum_{ x_i \in D } \frac{ \partial \Phi ( W,x_i+\eta_x \cdot \frac{ \partial \Phi(W,x_i) }{ \partial x_i } ) }{ \partial W } \Big|_{W = \wt{W}^{t-1}} 
\end{align*}
\end{definition}

We define gradients
\begin{definition}[gradient with respect to data]
\begin{align*}
    \frac{ \partial \Phi (\wh{W}^t,x_i) }{ \partial x_i } 
    = & ~ (f_{\wh{W}^t,a} (x_i) - y_i) \sum_{r=1}^m a_r \wh{w}^t_r \cdot \mathds{1}_{ x_i^\top \wh{w}^t_r \geq 0 } \\
    = & ~ \left( \sum_{r=1}^m a_r \phi ( x_i^\top \wh{w}_r^t ) - y_i \right) \cdot \sum_{r=1}^m a_r \wh{w}^t_r \cdot \mathds{1}_{ x_i^\top \wh{w}^t_r \geq 0 } \\
    = & ~ \left( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_r^t \cdot {\bf 1}_{ x_i^\top \wh{w}_r^t \geq 0 } - y_i \right) \cdot \sum_{r=1}^m a_r \wh{w}^t_r \cdot \mathds{1}_{ x_i^\top \wh{w}^t_r \geq 0 } \\
\end{align*}
and
\begin{align*}
    \frac{ \partial \Phi (\wt{W}^t,x_i) }{ \partial x_i } 
    = & ~ \left( f_{\wt{W}^t,a} (x_i) - y_i \right) \sum_{r=1}^m a_r \wt{w}^t_r \cdot \mathds{1}_{  x_i^\top \wt{w}^t_r \geq 0 } \\
     = & ~ \left( \sum_{r=1}^m a_r \cdot \phi( x_i^\top \wt{w}^t_r ) - y_i \right) \cdot \sum_{r=1}^m a_r \wt{w}^t \cdot {\bf 1}_{ x_i^\top \wt{w}_r^t \geq 0} \\
    = & ~ \left( \sum_{r=1}^m a_r \cdot x_i^\top \wt{w}^t_r \cdot {\bf 1}_{ x_i^\top \wt{w}^t_r \geq 0 } - y_i \right) \cdot \sum_{r=1}^m a_r \wt{w}^t \cdot {\bf 1}_{ x_i^\top \wt{w}_r^t \geq 0}
\end{align*}
\end{definition}

We then show either the positive result or the negative result.

\begin{lemma}[positive result]
There exist some generic constant $C_l$ and $C_u$ such that
\begin{align*}
\nbr{ \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} }_2 \leq C_u < C_l
 \leq \nbr{ \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} }_2.
\end{align*}
\Zhao{Sanjeev said 
\begin{align*}
\nbr{ \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} }_2 \geq C_u > C_l
 \geq \nbr{ \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} }_2.
\end{align*}
}
\end{lemma}

\begin{lemma}[negative result]
% Assume $\|\wt{w}_r-\wh{w}_r\|_2\leq \alpha \|\wt{w}_r\|_2$.
% Define $g(w)=\sum_{r=1}^m |a_r\cdot x_i^\top w_r|$. Let $c_1$ and $c_2$ satisfy that
% \begin{align*}
% g(\wt{w})\leq & ~ c_1\cdot | \sum_{r=1}^m a_r \cdot x_i^\top \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 } -y_i| \\
% g(\wh{w})\leq & ~ c_2\cdot | \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 } -y_i|.
% \end{align*}
% Define $h(w)=\sum_{r=1}^m \|a_r {w}_{r} \cdot {\bf 1}_{ x_i^\top {w}_{r} \geq 0}\|_2$.
% \begin{align*}
% h(\wt{w}) \leq & ~ c_3\cdot \|\sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\|_2,\\
% h(\wh{w}) \leq & ~ c_4\cdot \|\sum_{r=1}^m a_r \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0}\|_2.
% \end{align*}

Assume $\wt{w}_r \sim N(0,\sigma^2 I_d)$ and $a_r\sim N(0,1)$.

Let $\epsilon_t = $, for example $\epsilon_t = \frac{t}{ t + 1 }$. For each $r \in [m]$, $\| \wh{w}_r^t - \wt{w}_r^t \|_2 \leq R$ . We have 
\begin{align*}
\left\| \frac{\partial {\Phi} ( \tilde{W}^t,X ) }{\partial x_i} - \frac{\partial \Phi ( \hat{W}^t,X ) }{\partial x_i} \right\|_2 \leq \epsilon_t \cdot \left\| \frac{\partial \Phi ( \hat{W}^t,X ) }{\partial x_i} \right\|_2
\end{align*}
\end{lemma}
\begin{proof}
\Zhao{We need a proof for this.}

We define function $F: \R^{md} \times \R^{md} \times \R^{md} \times \R^{md} \times \R^{md} \rightarrow \R^d$ as follows
\begin{align*}
F(u_1,u_2,u_3,u_4) = \left( \sum_{r=1}^m a_r \cdot x_i^\top u_{1,r} \cdot {\bf 1}_{ x_i^\top u_{2,r} \geq 0 } - y_i \right) \cdot \sum_{r=1}^m a_r u_{3,r} \cdot {\bf 1}_{ x_i^\top u_{4,r} \geq 0}
\end{align*}
Then, we know that
\begin{align*}
\frac{\partial {\Phi} ( \tilde{W}^t,X ) }{\partial x_i} = F(\wt{W},\wt{W},\wt{W},\wt{W}) \\
\frac{\partial {\Phi} ( \hat{W}^t,X ) }{\partial x_i} = F(\wh{W},\wh{W},\wh{W},\wh{W})
\end{align*}
By triangle inequality, we can bound
\begin{align*}
 & ~ \| F(\wt{W},\wt{W},\wt{W},\wt{W}) - F(\wh{W},\wh{W},\wh{W},\wh{W}) \|_2 \\
= & ~ \| F(\wt{W},\wt{W},\wt{W},\wt{W}) - F(\wh{W},\wt{W},\wt{W},\wt{W}) \|_2 \\
& ~ + \| F(\wh{W},\wt{W},\wt{W},\wt{W}) - F(\wh{W},\wh{W},\wt{W},\wt{W}) \|_2  \\
& ~ + \| F(\wh{W},\wh{W},\wt{W},\wt{W}) - F(\wh{W},\wh{W},\wh{W},\wt{W}) \|_2 \\
& ~ + \| F(\wh{W},\wh{W},\wh{W},\wt{W}) - F(\wh{W},\wh{W},\wh{W},\wh{W}) \|_2 \\
= & ~ C_1 + C_2 + C_3 + C_4
\end{align*}



We bound these terms separately. We first upper bound $C_1$,
\begin{align*}
    C_1 = & \| F(\wt{W},\wt{W},\wt{W},\wt{W}) - F(\wh{W},\wt{W},\wt{W},\wt{W}) \|_2\\
    =&\left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 }-\sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 } \right) \cdot \sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\right\|_2\\
    = & ~ \left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top (\wt{w}_{r}-\wh{w}_{r}) \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 } \right) \cdot \sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\right\|_2\\
    = & ~ \left| \sum_{r=1}^m a_r \cdot x_i^\top (\wt{w}_{r}-\wh{w}_{r}) \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 } \right|\cdot \left\| \sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0} \right\|_2\\
\end{align*}
Notice that $x_i^\top \wt{w}_{r}$ follows normal distribution $N(0,\sigma^2\|x_i\|_2^2)$.
Let $P_i=\{r\in [m]:x_i^\top \wt{w}_{r}\geq 0\}$,
then by Chernoff Bound we have
$
\Pr[\left||P_i|-\frac{m}{2}\right|\geq \frac { \epsilon} {2}m]\leq 2e^{-\frac {\epsilon^2} 2}
$.
Let $\mathcal{E}_1$ be the event that $|P_i|\leq \frac {1+\epsilon}{2}m$.
Let $v=\sum_{r\in P_i}a_r \wt{w}_{r}$,
then $v_j= \sum_{r\in P_i}a_r \cdot(\wt{w}_{r})_j$.
Hence $\E[v_j]=0$,
and 
\[
\E[v_j^2]=\sum_{r\in P_i}\E[a_r^2 \cdot(\wt{w}_{r})_j^2]=|P_i|\sigma^2,
\]
and
\begin{align*}
    \E[v_j^4]&=\sum_{r\in P_i}\E[a_r^4 \cdot(\wt{w}_{r})_j^4]+\sum_{r_1,r_2\in P_i, r_1\neq r_2}\E[a_{r_1}^2a_{r_2}^2 \cdot(\wt{w}_{r_1})_j^2(\wt{w}_{r_2})_j^2]\\
    &=9|P_i|\sigma^4+3|P_i|(|P_i|-1)\sigma^4\\
\end{align*}
where we use the fact that $\E_{X\sim N(0,\sigma^2)}[X^4]=3\sigma^4$.
Then we have $\mathbf{Var}[v_j^2]= \E[v_j^4]-\E[v_j^2]^2=2|P_i|(|P_i|+3)\sigma^2$.
Hence by Chebyshev inequality we have 
\[\Pr[v_j^2\geq |P_i|\sigma^2+\delta\cdot 2|P_i|\sigma^2]\leq \frac 1 {\delta^2}.
\]
\textcolor{red}{Chebyshev is very loose, but I cannot think of sharper bound here}
Let $\mathcal{E}_2$ be the event that $\forall j\in [d]$, $v_j^2\geq |P_i|\sigma^2+\delta\cdot 2|P_i|\sigma^2$.

If both $\mathcal{E}_1$ and $\mathcal{E}_2$ happen,
then 
\[
\left\| \sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0} \right\|_2\leq d\cdot (2\delta+1)\sigma^2 \cdot \frac {1+\epsilon}2 m
\]
This will happen with probability at least $1-2e^{-\frac {\epsilon^2}2}-d/{\delta^2}$.

Now let us look at the term $ \left| \sum_{r=1}^m a_r \cdot x_i^\top (\wt{w}_{r}-\wh{w}_{r}) \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 } \right|$.
Let $y_r=x_i^\top (\wt{w}_{r}-\wh{w}_{r})$,
then by the assumption on $\wh{w}_r$ we have $|y_r|\leq R$.
Fix $\{y_r\}_{r=1}^m$.
Then $ \sum_{r=1}^m a_r \cdot x_i^\top (\wt{w}_{r}-\wh{w}_{r}) \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 } =\sum_{r\in P_i} a_ry_r$,
which follows the distribution $N(0,\sum_{r\in P_i}y_r^2)$.
Let $t=\sum_{r\in P_i}y_r^2\leq |P_i|\cdot R^2$.
From the tail bound of normal distribution,
we have for $k>1$,
\[
\Pr_{X\sim N(0,t)}[|X|\geq k\sqrt{t}]\leq e^{-{k^2}/2}
\]
Let $\mathcal{E}_3$ be the event that $|\sum_{r\in P_i} a_ry_r|\leq k\sqrt{|P_i|R^2}$.
Then when both $\mathcal{E}_1$ and $\mathcal{E}_3$ happen,
we have
\[
\left| \sum_{r=1}^m a_r \cdot x_i^\top (\wt{w}_{r}-\wh{w}_{r}) \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 } \right|\leq  k\sqrt{\frac{(1+\epsilon)mR^2}2}.
\]
This will happen with probability at least $1-2e^{-\frac {\epsilon^2}2}-e^{-{k^2}/2}$.






We can upper bound $C_2$ in the following way,
\begin{align*}
    C_2
    = & ~ \| F(\wh{W},\wt{W},\wt{W},\wt{W}) - F(\wh{W},\wh{W},\wt{W},\wt{W}) \|_2\\
    = & ~ \left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 }-\sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 } \right) \cdot \sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\right\|_2\\
    = & ~ \left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot ({\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0 }-{\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 }) \right) \cdot \sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\right\|_2\\
    \leq & ~ g(\wh{w}) \cdot \left\| \sum_{r=1}^m a_r \wt{w}_{r}\cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\right\|_2 \\
    \leq & ~ c_2\cdot \|F(\wh{W},\wh{W},\wt{W},\wt{W})\|_2
\end{align*}
\textcolor{red}{may be better to take expectation on the first term}

We can upper bound $C_3$,
\begin{align*}
    C_3
    = & ~ \| F(\wh{W},\wh{W},\wt{W},\wt{W}) - F(\wh{W},\wh{W},\wh{W},\wt{W}) \|_2\\
    = & ~ \left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 } -y_i\right) \cdot \left(\sum_{r=1}^m a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0} - \sum_{r=1}^m a_r \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\right)\right\|_2\\
    = & ~ \left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 } -y_i\right) \cdot \sum_{r=1}^m a_r (\wt{w}_{r}-\wh{w}_{r}) \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0} \right\|_2\\
    \leq & ~ \alpha \left|( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 }-y_i )\right|\cdot \sum_{r=1}^m \|a_r \wt{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0}\|_2 \\
    \leq & ~ \alpha \cdot c_3 \cdot \|F(\wh{W},\wh{W},\wt{W},\wt{W})\|_2
\end{align*}

\begin{align*}
    C_4
    = & ~ \| F(\wh{W},\wh{W},\wh{W},\wt{W}) - F(\wh{W},\wh{W},\wh{W},\wh{W}) \|_2\\
    = & ~ \left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 } -y_i\right) \cdot \left(\sum_{r=1}^m a_r \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0} - \sum_{r=1}^m a_r \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0}\right)\right\|_2\\
    = & ~ \left\|\left( \sum_{r=1}^m a_r \cdot x_i^\top \wh{w}_{r} \cdot {\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0 } -y_i\right) \cdot \sum_{r=1}^m a_r \wh{w}_{r} \cdot ({\bf 1}_{ x_i^\top \wt{w}_{r} \geq 0} -{\bf 1}_{ x_i^\top \wh{w}_{r} \geq 0})\right\|_2 \\
    \leq & ~c_4\cdot \|F(\wh{W},\wh{W},\wh{W},\wh{W})\|_2
\end{align*}


\end{proof}

A stronger claim is to look at the inner products of the gradient and the input
\begin{align*}
| x_i^\top \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} |
~~~\text{and}~~~~
| x_i^\top \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} |.
\end{align*}

We then show either the positive result or the negative result.

\begin{lemma}[positive result]
There exist some generic constant $C_l$ and $C_u$ such that
\begin{align*}
| x_i^\top \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} | \leq C_u < C_l
 \leq | x_i^\top \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} |.
\end{align*}
\end{lemma}

\begin{lemma}[negative result]
%Negative result $\|\frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i}\|_2 \approx \|\frac{\partial \Phi ( \hat{W},X ) }{\partial x_i}\|_2$. One possible argument: 
Let $\epsilon_t = $, for example $\epsilon_t = \frac{t}{ t + 1 }$. We have 
\begin{align*}
\nbr{ x_i^\top \frac{\partial {\Phi} ( \tilde{W}^t,X ) }{\partial x_i} - x_i^\top \frac{\partial \Phi ( \hat{W}^t,X ) }{\partial x_i} }_2 \leq \epsilon_t \cdot \nbr{ x_i^\top \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} }_2
\end{align*}
%. Also see the value $\|\frac{\partial {\Phi}( \tilde{W},X ) }{\partial x_i}\|_2$ and $\|\frac{\partial \Phi ( \hat{W},X ) }{\partial x_i}\|_2$.
\end{lemma}

\begin{lemma}[positive result]
There exist some generic constant $C_l$ and $C_u$ such that
\begin{align*}
| ( \tilde{x}_i - x_i )^\top \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} | \leq C_u < C_l
 \leq | ( \tilde{x}_i - x_i )^\top \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} |.
\end{align*}
\end{lemma}

\begin{lemma}[positive result]
There exist some generic constant $C_l$ and $C_u$ such that
\begin{align*}
| ( \Pi(x_i) - x_i )^\top \frac{\partial \Phi ( \hat{W},X ) }{\partial x_i} | \leq C_u < C_l
 \leq | ( \Pi(x_i) - x_i )^\top \frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i} |.
\end{align*}
\end{lemma}


\begin{lemma}[Extension of Theorem 4.1 in \cite{dzps19}]
Under the same conditions as in Theorem 4.1 in \cite{dzps19} for adversarial training, we have
\begin{align*}
\Phi^{(k+1)} \leq ( 1 - \frac{\eta \lambda_0}{2} ) \cdot \Phi^{(k)} + C.
\end{align*}
\end{lemma}
\begin{proof}
Some ideas about $C$. For a large perturbation of $x_i$, we have $\nbr{H^{(k)} - H^{(0)}}_2 \leq \frac{4n^2 R^*}{\sqrt{2\pi}\delta} \leq \frac{4n^2 R}{\sqrt{2\pi}\delta} + C_1$, where $R^*$ is much lager than $R$ in \cite{dzps19}. Plug this into the proof of Theorem 4.1, on page 9 bottom part of \cite{dzps19} and get 
\begin{align*}
\Phi^{(k+1)} \leq ( 1 - \frac{\eta \lambda_0}{2} ) \cdot \Phi^{(k)} + C.
\end{align*}
\end{proof}

%\subsection{Large Deviation of Input Data}

%Show that when $\nbr{x - \tilde{x}}_2$ is large, then 

%\subsection{Discussions}
%\Zhao{Some possible TODO in the future, Either say positive result: $\|\frac{\partial {\Phi} ( \tilde{W},X ) }{\partial x_i}\|_2 \geq \tilde{g} > g \geq \|\frac{\partial \Phi ( \hat{W},X ) }{\partial x_i}\|_2$.}



==> backup.tex <==
\begin{definition}[Step function]\label{def:step_function}
Given parameters $r \in [0,2],\delta \in [0,2]$ and $\epsilon \in [0,1]$.
A uni-variate function $p:[0, 2]\rightarrow\R$ is a $(r, \delta, \epsilon)$ step function if it satisfies the following two properties:
\begin{enumerate}
    \item $\forall x\in[0, ~r], ~~|p(x)-1|\leq\epsilon$
    \item $\forall x\in[r + \delta, ~2], ~~|p(x)|\leq\epsilon$
\end{enumerate}
.
\end{definition}

\begin{lemma}
\label{lem:poly-step}
For every $~r,~\delta > 0$ with $r + \delta\leq 2$, there exists a polynomial $p(x)=\sum_{i=0}^k\beta_ix^i$ with degree $k=\Theta(\delta^{-2} \log(1/ \epsilon ))$ and $|\beta_i|\leq 2^{O(k)}$ that is a $(r, \delta, \epsilon)$ step function (Definition~\ref{def:step_function}). Furthermore
\end{lemma}
\begin{proof}
According to Corollary 5.4 in~\cite{frostig2016principal}, the following polynomial
\begin{align*}
    p_0(x)=\sum_{i=0}^k  x(1-x^2)^i \prod_{j=1}^i (1 - 1/(2j) ) 
\end{align*}
with $k= \lceil 16 \delta^{-2} \log(1/\epsilon) \rceil$ is an $\epsilon-$approximation to the $\text{sign}(\cdot)$ function on $[-1,1]\textbackslash [- \delta/4, \delta/4]$, e.g.
\begin{enumerate}
    \item $\forall x\in[\delta/4,~1], ~~|p(x)-1|\leq\epsilon$
    \item $\forall x\in[-1,~-\delta/4], ~~|p(x)+1|\leq\epsilon$
\end{enumerate}
.
We set $R=\max\{ r + \delta/2, 2 - (r+ \delta / 2 )\}$ and it's clear that $1\leq R\leq 2$. Then for every $x\in[0,2]$, we know $( x - r - \delta / 2 )/R \in[-1,1]$. Therefore the following function 
\begin{align*}
    p(x) = \frac{1}{2} - \frac{1}{2} \cdot p_0  \left(\frac{x - r -  \delta/2 }{R}\right)
\end{align*}
satisfies the desired properties. If we express $b$ as $\sum_{i=0}^k \beta_i x^i$, then we can bound the coefficients as follows
\begin{align*}
    |\beta_i|\leq O(1) \cdot  {k\choose k/2} \cdot (1/R)^k  = 2^{O(k)}
\end{align*}.
\end{proof}


\begin{lemma}
Given a dataset $S=\{(x_i, y_i)_{i=1}^n\}$ of $n$ examples, and a $(r^2, ~\delta^2+2\delta r, ~\frac{\epsilon}{2n})$ step function (Definition~\ref{def:step_function}) $p$ realized by the degree $\Theta((\delta^4\log(n/\epsilon))$ polynomial given by lemma~\ref{lem:poly-step}, the following function
\begin{align*}
    f^*(x) = \sum_{i=1}^n y_i \cdot p(\|x - x_i\|_2^2)
\end{align*}
has $\epsilon$ robust loss on $S$, i.e. $L(f, S, r)\leq\epsilon/2$
\end{lemma}
\begin{proof}
For any $(x_i, y_i)\in S$, it is clear from the properties of $p$ that 
\begin{align*}
\forall x\in B(x_i, r), |f^*(x)-y_i| \leq \sum_{i=1}^n |y_i| \cdot (\epsilon/(2n)) \leq\frac{\epsilon}{2} 
\end{align*}
It follows that $L(f,S,r)\leq\epsilon$ by the 1-Lipschitzness of the loss function $l$.
\end{proof}

\begin{lemma}
There exists an one layer pseudo-net $f_{W^*}(x)=\frac{1}{\sqrt{m}}\sum_{i=1}^m a_i {w_i^*}^\top x \ind_{{w_i^*}^\top x + b_i \geq 0}$ with $m\geq (2nL/\epsilon)^{\frac{1}{\delta^2}}$ and $\|W^*\|_F \leq (2nL/\epsilon)^{\frac{1}{\delta^2}}$ such that
\begin{align*}
    \max_{x\in B(0,1)} |f^*(x) - f_{W^*}(x)| \leq \epsilon/2
\end{align*}
and therefore $L(f_{W^*}, S, r)\leq\epsilon$.
\end{lemma}
\begin{proof}
TODO
\end{proof}

==> convergence.tex <==
\subsection{Convergence}
\label{sec:converge}




\Orestis{todo: 1. lemma+definition seem out of nowhere->set the stage, say what you will do. 2. missing definition of gradient and pseudonet gradient 3. $W^*$ undefined 4. $a_r~\{\pm 1/m^{1/3}\}$ 5. Initialization is $W^{ij}\sim N(0,1/m)$ 6.In my part I have written $\ind\{abc\}$ instead of $\ind_{abc}$}

\Orestis{missing notation: S(t), $\tilde{\ell}$, write guarantee for $min_t$ as in the other paper. Missing definition of pseudoloss}
\Yi{w.h.p. of initilization}
\begin{theorem}

\end{theorem}
\begin{proof}
For simplicity, in the proof we use the following shorthand notations to denote various distances.
\begin{itemize}[noitemsep,topsep=0pt]
    \item[] $D_{\text{max}}:= \max_{ t \in [T] }\|W^{(t)} - W^{(0)}\|_{2,\infty}$
    \item[] $D_{W^{*}}:= \|W^{*} - W^{(0)}\|_{2,\infty}$
\end{itemize}
By condition, we know $D_{W^*}=O\left(\frac{R}{m^{2/3}}\right)$.
Even though in Algorithm~\ref{alg:adv-train} the parameters $W$ are updated using the gradients of the \emph{real net}, in this proof we consider the pseudo-net as the object being optimized. Thus we need to relate the real net gradients to the pseudo-net gradients. For ease of presentation, we define the following convenient notations for the two notions of gradients:
\begin{itemize}[noitemsep,topsep=0pt]
    \item[] real net gradient $\nabla^{(t)}:=\nabla_W\mathcal{L}(f(W^{(t)}), S^{(t)})$ 
    \item[] pseudo-net gradient $\hat{\nabla}^{(t)}:=\nabla_W\mathcal{L}(g(W^{(t)}), S^{(t)})$
\end{itemize}
In fact, by Lemma~\ref{lemma:coupling}, we know that they are coupled w.h.p. as long as $W^{(t)}$ stays close to initialization (i.e., $D_{\max}\leq m^{-7/12}$).
\begin{align*}
      \| \hat{\nabla}^{(t)} - \nabla^{(t)} \|_{2,1} \leq O\left(Lnm^{7/12}\right) \| W^{(t)} - W^{(0)}\|_{2,\infty}
\end{align*}
\begin{remark}
We assume for now $D_{\max}\leq m^{-7/12}$ is true and in the end we will set proper values for $T, \eta$ and $m$ to make sure this is indeed the case.
\end{remark}
Furthermore we note there is an upper bound on the gradient size:
\begin{align}\label{ineq:gradient-size}
    \|\nabla^{(t)}_r\|_2 &\leq L |a_r| \left(\frac{1}{n}\sum_{i=1}^n \sigma'\left(\inner{W^{(t)}_r}{x_i}+b_r^{(0)}\right)\|x_i\|_2\right) \notag\\
    &\leq \frac{L}{m^{1/3}}
\end{align}

Due to the linearity of $g$ with respect to $W$, the loss $\mathcal{L}(g(W), S)$ is in fact convex in $W$. We proceed to exploit the convexity and swap in the real net gradient:
\begin{align*}
    & ~ \mathcal{L}(g(W^{(t)}), S^{(t)}) - \mathcal{L}(g(W^*), S^{(t)}) \\
    \leq & ~\inner{\nabla^{(t)}}{W^{(t)} - W^*} + \inner{\hat{\nabla}^{(t)} - \nabla^{(t)}}{W^{(t)} - W^*} \\
    \leq & ~ \underbrace{\inner{\nabla^{(t)}}{W^{(t)} - W^*}}_{:=\text{\textalpha}^{(t)}}  \\
    &~~~~~~~~~~~~~~~~~~~~+ \underbrace{\|\hat{\nabla}^{(t)} - \nabla^{(t)}\|_{2,1}\|W^{(t)} - W^* \|_{2,\infty}}_{:=\text{\textbeta}^{(t)}}
\end{align*}
Then we deal with \textalpha~and~\textbeta~terms separately. As for the former, we use the standard online gradient descent proof technique:
\begin{align*}
\text{\textalpha}^{(t)} &\leq \frac{\eta}{2} \| \nabla^{(t)} \|_F^2 + \frac{\| W^{(t)} - W^* \|_F^2 - \| W^{(t+1)} - W^* \|_F^2}{2\eta} 
\end{align*}
We then sum over time indices $t$ and take care of the telescopic terms:
\begin{align*}
\sum_{t=1}^T \text{\textalpha}^{(t)} &\leq \frac{\eta}{2}\left(\sum_{t=1}^T\|\nabla^{(t)}\|_F^2\right) + \frac{\| W^* -  W^{(0)}\|_F^2}{2\eta} \\
&\leq \frac{\eta L^2 m^{1/3}}{2}T + \frac{m D_{W^*}^2}{2\eta}
\end{align*}
where we used the fact $\|W^* -  W^{(0)}\|_F^2\leq m\cdot \|W^* -  W^{(0)}\|_{2,\infty}=m D_{W^*}^2$ 
as well as $\|\nabla^{(t)}\|_F^2\leq \sum_{r=1}^m \|\nabla_r^{(t)}\|_2^2\leq L^2m^{1/3}$.

For the $\text{\textbeta}^{(t)}$'s, we first invoke Lemma~\ref{lemma:coupling} and then apply a simple triangle inequality:
\begin{align*}
\text{\textbeta}^{(t)} &\leq O\left(Lnm^{7/12}\right)\| W^{(t)} - W^* \|_{2,\infty}\\
&\leq O\left(Lnm^{7/12}\right) \left(D_{\text{max}} + D_{W^{*}}\right)
\end{align*}

Furthermore we can bound the size of $D_{\text{max}}$ using the bound on gradients, i.e. $\|\nabla^{(t)}_r\|_2\leq Lm^{-1/3}$ using Inequality~\ref{ineq:gradient-size}.
\begin{align*}
    D_{\text{max}} &= \max_{ t \in [T]}\|W^{(0)} - W^{(t)}\|_{2,\infty} \\
    &\leq \sum_{t=1}^T \eta \max_{r\in[m]}\|\nabla^{(t)}_r\|_2 \leq \frac{\eta L T}{m^{1/3}}
\end{align*}

Putting it together with the condition $D_{W*}=O\left(\frac{R}{m^{2/3}}\right)$ that we already have, we obtain the following:
\begin{align*}
    & ~ \sum_{t=1}^T  \mathcal{L}(g(W^{(t)}), S^{(t)}) - \sum_{t=1}^T \mathcal{L}(g(W^*), S^{(t)})\\ 
    \leq & \sum_{t=1}^T \text{\textalpha}^{(t)} + \sum_{t=1}^T \text{\textbeta}^{(t)} \\
    \leq & O\left(\eta L^2 T n m^{1/4} + \frac{\eta R L T n}{m^{1/12}}  +  m^{1/3} \eta L^2 T +  \frac{R^2}{m^{1/3} \eta}\right)
\end{align*}

Finally we arrive at the desired statement
\begin{align*}
   \frac{1}{T} \sum_{t=1}^T \mathcal{L}(g(W^{(t)}), S^{(t)}) - \frac{1}{T} \sum_{t=1}^T \mathcal{L}(g(W^*), S^{(t)}) &\leq \varepsilon
\end{align*}
if we set the hyper-parameters $T, m, \eta$ to be the following:
\begin{itemize}
    \item[] $T=\Theta( \epsilon^{-2} L^2R^2 )$,
    \item[] $m=\Omega\left(\max\left\{ \left(\frac{n}{\epsilon}\right)^{12}, \left(\frac{Rn}{L\epsilon}\right)^{12/5}, \left(\frac{R^2L}{\epsilon}\right)^{12} \right\} \right)$,
    \item[] $\eta=\frac{R}{m^{1/3} L \sqrt{T}}=\Theta(m^{-1/3} L^{-2} \epsilon )$  
\end{itemize}
Note the the requirement on $m$ is to satisfy $\eta L^2 T n m^{1/4} + \frac{\eta R L T n}{m^{1/12}} \leq O(\epsilon)$ and $D_{\max}\leq m^{-7/12}$
.


\end{proof}

==> preli.tex <==
\section{Preliminaries}


\subsection{Probability tools}



\begin{theorem}[Chernoff bound]\label{thm:chernoff}
Let $X = \sum_{i=1}^n X_i$, where $X_i=1$ with probability $p_i$ and $X_i = 0$ with probability $1-p_i$, and all $X_i$ are independent. Let $\mu = \E[X] = \sum_{i=1}^n p_i$. Then \\
1. $ \Pr[ X \geq (1+\delta) \mu ] \leq \exp ( - \delta^2 \mu / 3 ) $, $\forall \delta > 0$ ; \\
2. $ \Pr[ X \leq (1-\delta) \mu ] \leq \exp ( - \delta^2 \mu / 2 ) $, $\forall 0 < \delta < 1$. 
\end{theorem}

\begin{theorem}[Hoeffding bound]\label{thm:hoeffding}
Let $X_1, \cdots, X_n$ denote $n$ independent bounded variables in $[a_i,b_i]$. Let $X= \sum_{i=1}^n X_i$, then we have
\begin{align*}
\Pr[ | X - \E[X] | \geq t ] \leq 2\exp \left( - \frac{2t^2}{ \sum_{i=1}^n (b_i - a_i)^2 } \right)
\end{align*}
\end{theorem}

\begin{theorem}[Bernstein inequality]
Let $X_1, \cdots, X_n$ be independent zero-mean random variables. Suppose that $|X_i| \leq M$ almost surely, for all $i$. Then, for all positive $t$,
\begin{align*}
\Pr \left[ \sum_{i=1}^n X_i > t \right] \leq \exp \left( - \frac{ t^2/2 }{ \sum_{j=1}^n \E[X_j^2]  + M t /3 } \right).
\end{align*}
\end{theorem}


\begin{theorem}[anti-concentration of Gaussian distribution]
Let $X\sim N(0,\sigma^2)$,
that is,
the probability density function of $X$ is given by $\phi(x)=\frac 1 {\sqrt{2\pi\sigma^2}}e^{-\frac {x^2} {2\sigma^2} }$.
Then
\begin{align*}
    \Pr[|X|\leq t]\in \left( \frac 2 3\frac t \sigma, \frac 4 5\frac t \sigma \right).
\end{align*}
\end{theorem}

\begin{lemma}[Lemma 1 on page 1325 of Laurent and Massart]\label{lem:chi_square_tail}
Let $X \sim {\cal X}_k^2$ be a chi-squared distributed random variable with $k$ degrees of freedom. Each one has zero mean and $\sigma^2$ variance. Then
\begin{align*}
\Pr[ X - k \sigma^2 \geq ( 2 \sqrt{kt} + 2t ) \sigma^2 ] \leq \exp (-t) \\
\Pr[ k \sigma^2 - X \geq 2 \sqrt{k t} \sigma^2 ] \leq \exp(-t)
\end{align*}
\end{lemma}



\begin{algorithm}[!t]\caption{The algorithm being used in \cite{mmstv18}.}
\begin{algorithmic}[1]
\Procedure{\textsc{MadryAlgorithm}}{$\{ (x_i, y_i) \}_{i \in [n]}$}
	\State $D^{0} \leftarrow \{ x_1, x_2, \cdots, x_n \}$
	\State $W^{0} \leftarrow \N(0,I)$
	\State $t \leftarrow 1$
	\While{}
		\State $D^t \leftarrow \emptyset$
		\For{$i=1 \to 100$}
			\State Sample $x_i \sim D^{0}$
			\State $\wt{x}_i \leftarrow x_i + \eta_x \cdot \frac{ \partial \Phi(W,x_i,y_i) }{ \partial x_i }$
			\State $D^t \leftarrow D^t \cup \{ \wt{x}_i  \}$
		\EndFor
		%\State Sample $x \sim D^{t-1}$
		\State $W^{t} \leftarrow W^{t-1} - \eta_w \cdot \sum_{x_i \in D^t} \frac{ \partial \Phi(W,x_i.y_i) }{ \partial W }$
	\EndWhile
\EndProcedure
\end{algorithmic}\caption{}
\end{algorithm}


\subsection{Problem formulation}

We consider a two-layer ReLU activated neural network with $m$ neurons in the hidden layer:
\begin{align*}
f_{W,a} (x) =  \sum_{r=1}^m a_r \sigma ( w_r^\top x )
\end{align*}
where $x \in \R^d$ is the input, $w_1, \cdots, w_m \in \R^d$ are weight vectors in the first layer, $a_1, \cdots, a_m \in \R$ are weights in the second layer (we hide $1/\sqrt{m}$ in $a_i$s). 

We can compute gradient of $f_{W,a}(x)$ 
\begin{align*}
\frac{ \partial f_{W,a} (x) }{ \partial x } =  \sum_{r=1}^m a_r w_r \cdot \mathds{1}_{ w_r^\top x \geq 0 }
\end{align*}


We define objective function $\Phi$ as follows
\begin{align*}
\Phi (W,X,Y) = \frac{1}{2} \sum_{i=1}^n ( y_i - f_{W,a} (x_i) )^2
\end{align*}
For simplicity, we will use $\Phi(W,X)$ to denote $\Phi(W,X,Y)$ in the rest of the proofs, since $Y$ never changed.

We can compute the gradient of $\Phi$ in terms of $x_i$
\begin{align*}
\frac{ \partial \Phi(W,X,Y) }{ \partial x_i } = & ~ ( f_{W,a} (x_i) - y_i ) \cdot \frac{ \partial f_{W,a} (x_i) }{ \partial x_i } \\
= & ~ ( f_{W,a} (x_i) - y_i ) \cdot \left( \sum_{r=1}^m a_r w_r \cdot \mathds{1}_{w_r^\top x_i \geq 0 }  \right) \\
= & ~ \left( \sum_{r=1}^m a_r \sigma(w_r^\top x_i) - y_i \right) \cdot \left( \sum_{r=1}^m a_r w_r \cdot \mathds{1}_{w_r^\top x_i \geq 0 }  \right)
\end{align*}


Given $\{ x_i \}_{i \in [n]}$, we define the following Gram matrix $H^{\infty} \in \R^{n \times n}$ as follows:
\begin{align*}
H_{i,j}^{\infty} = & ~ \E_{w \sim \N(0,I)} \left[ x_i^\top x_j \mathds{1}_{ w^\top x_i \geq 0, w^\top x_j \geq 0 } \right].
\end{align*}
Then it is easy to see that
\begin{align*}
H_{i,j}^{\infty} = & ~ x_i^\top x_j \E_{w \sim \N(0,I)} \left[ \mathds{1}_{ w^\top x_i \geq 0, w^\top x_j \geq 0 } \right] \\
= & ~  x_i^\top x_j \frac{  ( \pi - \text{arc}\cos (x_i^\top x_j) ) }{ 2\pi }
\end{align*}

Let $\wt{x}_i \in \R^d$ be defined as 
\begin{align*}
\wt{x}_i = x_i + \epsilon \cdot \frac{ \partial \Phi(W,X) }{ \partial x_i } = x_i + \delta_{x,i}.
\end{align*}

We can write $\wt{H}_{i,j}^{\infty}$,
\begin{align*}
\wt{H}_{i,j}^{\infty} 
= & ~ \E_{ w \sim \N(0,I) } \left[ \wt{x}_i^\top \wt{x}_j \mathds{1}_{ w^\top \wt{x}_i \geq 0 , w^\top \wt{x}_j \geq 0 } \right] \\
= & ~ \E_{ w \sim \N(0,I) } \left[ (x_i + \delta_{x,i} )^\top ( x_j + \delta_{x,j} ) \mathds{1}_{ w^\top (x_i + \delta_{x,i} ) \geq 0 , w^\top (x_j + \delta_{x,j}) \geq 0 } \right]
\end{align*}



\begin{lemma}[General version of Lemma 3.1]
\Zhao{Unfinished....}
If $m = \Omega(  )$, we have 
\begin{align*}
\| H(0) - H^{\infty} \|_2 \leq \frac{ \lambda_0 }{4}, \mathrm{~and~} \lambda_{\min} ( H(0) ) \geq \frac{3}{4} \lambda_0.
\end{align*}
hold with probability at least $1-\delta$.
\end{lemma}

We restate the original version of Lemma 3.2 in \cite{dzps19},
\begin{lemma}[perturbed $w$, Lemma 3.2 in \cite{dzps19}]
Let $R = \frac{ c \delta \lambda_0 }{ n^2 }$. 
If $\wt{w}_1, \cdots, \wt{w}_m$ are i.i.d. generated ${\cal N}(0,I)$, then with probability at least $1-\delta$, the following holds. For any set of weight vectors $w_1, \cdots, w_m \in \R^d$ that satisfy for any $r\in [m]$, $\| \wt{w}_r - w_r \|_2 \leq R$ for some small positive constant $c$, then the matrix $H \in \R^{n \times n}$ defined
\begin{align*}
    H_{i,j} (x, w) = & ~ \frac{1}{m} x_i^\top x_j \sum_{r=1}^m \mathds{1}_{ w_r^\top x_i \geq 0, w_r^\top x_j \geq 0 } \\
    H_{i,j} (x, \wt{w}) = & ~ \frac{1}{m} x_i^\top x_j \sum_{r=1}^m \mathds{1}_{ \wt{w}_r^\top x_i \geq 0 , \wt{w}_r^\top x_j \geq 0}
\end{align*}
Then we have
\begin{align*}
\| H (x,w) - H(x,\wt{w}) \|_2 < \frac{1}{4} \lambda_0, \mathrm{~~~and~~~} \lambda_{\min} ( H  ) > \frac{1}{2} \lambda_0.
\end{align*}
\end{lemma}
For the completeness, we still provide the proof here.
\begin{proof}
For simplicity, let $\wt{H} = H(x,\wt{w})$ and let $H = H(x,w)$.


We define the event
\begin{align*}
A_{i,r} = \left\{ \exists u : \| u - \wt{w}_r \|_2 \leq R, {\bf 1}_{ x_i^\top \wt{w}_r \geq 0 } \neq {\bf 1}_{ x_i^\top u \geq 0 } \right\}.
\end{align*}
Note this event happens if and only if $| \wt{w}_r^\top x_i | < R$. Recall that $\wt{w}_r \sim \N(0,I)$. By anti-concentration inequality of Gaussian, we have
\begin{align*}
\Pr[ A_{ir} ] = \Pr_{ z \sim \N(0,1) } [ | z | < R ] \leq \frac{ 2 R }{ \sqrt{2\pi} }.
\end{align*}
Therefore, for any set of weight vectors $w_1, \cdots, w_m$ that satisfy the assumption in the Lemma, we can bound the entry-wise deviation on their induced matrix $H$, 
\begin{align*}
\E[ | \wt{H}_{i,j} - H_{i,j} | ] 
= & ~ \E \left[ \frac{1}{m} \left| x_i^\top x_j \sum_{r=1}^m ( {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } ) \right| \right] \\
\leq & ~ \frac{1}{m} \sum_{r=1}^m \E[  {\bf 1}_{ A_{ir} \cup A_{jr} } ] \\
\leq & ~ \frac{4 R}{ \sqrt{2\pi} } 
\end{align*} 

Summing over $(i,j)$, we have
\begin{align*}
\E[ \| H - \wt{H} \|_1 ] = \E \left[ \sum_{i=1}^n \sum_{j =1}^n | H_{i,j} - \wt{H}_{i,j} | \right] \leq \frac{4 n^2 R}{  \sqrt{2\pi} }.
\end{align*}
Thus by Markov's inequality, we have
\begin{align*}
\Pr \left[ \| H - \wt{H} \|_1  \leq \frac{4 n^2 R}{  \sqrt{2\pi}  \delta } \right] \geq 1-\delta.
\end{align*}
Next, we use matrix perturbation theory to bound the deviation from the initialization
\begin{align*}
\| H - \wt{H} \|_2 \leq \| H - \wt{H} \|_F \leq \| H - \wt{H} \|_1 \leq \frac{ 4 n^2 R }{ \sqrt{2\pi} \delta }.
\end{align*}
Lastly, we lower bound the smallest eigenvalue by plugging in $R$
\begin{align*}
\lambda_{\min} (H) \geq \lambda_{\min} ( \wt{H} ) - \frac{4 n^2 R}{ \sqrt{2\pi} \delta } \geq \frac{ \lambda_0 }{2}
\end{align*}
\end{proof}

We improve the probability dependence in original proof

\begin{lemma}[perturbed $w$, high probability, Lemma 3.2 in \cite{dzps19}]
Let $R = \frac{ c \lambda_0 }{ n^2 }$. 
If $\wt{w}_1, \cdots, \wt{w}_m$ are i.i.d. generated ${\cal N}(0,I)$, then with probability at least $1-\exp(-\Omega(mR))$, the following holds. For any set of weight vectors $w_1, \cdots, w_m \in \R^d$ that satisfy for any $r\in [m]$, $\| \wt{w}_r - w_r \|_2 \leq R$ for some small positive constant $c$, then the matrix $H \in \R^{n \times n}$ defined
\begin{align*}
    H_{i,j} (x, w) = & ~ \frac{1}{m} x_i^\top x_j \sum_{r=1}^m \mathds{1}_{ w_r^\top x_i \geq 0, w_r^\top x_j \geq 0 } \\
    H_{i,j} (x, \wt{w}) = & ~ \frac{1}{m} x_i^\top x_j \sum_{r=1}^m \mathds{1}_{ \wt{w}_r^\top x_i \geq 0 , \wt{w}_r^\top x_j \geq 0}
\end{align*}
Then we have
\begin{align*}
\| H (x,w) - H(x,\wt{w}) \|_2 < \frac{1}{4} \lambda_0,% \mathrm{~~~and~~~} \lambda_{\min} ( H  ) > \frac{1}{2} \lambda_0.
\end{align*}
\end{lemma}
\begin{proof}
\Zhao{Working on it now.}

We random variable we care is
\begin{align*}
\sum_{i} \sum_j | \wt{H}_{i,j} - H_{i,j} | 
= & ~ \frac{1}{m} \sum_{i=1}^n \sum_{j=1}^n \left| x_i^\top x_j \sum_{r=1}^m ( {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } ) \right|  \\
\leq & ~ \frac{1}{m} \sum_{i=1}^n \sum_{j=1}^n \sum_{r=1}^m \left| {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right| \\
= & ~ \frac{1}{m} \sum_{r=1}^m  \sum_{i=1}^n \sum_{j=1}^n \left| {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right|
\end{align*}


Define $s_r=\sum_{i=1}^n \sum_{j=1}^n\left| {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right|$.
Then $s_r$ is a random variable that only depends on $\wt{w}_r$.
Since $\{\wt{w}_r\}_{r=1}^m$ are independent,
$\{s_r\}_{r=1}^m$ are also mutually independent.

If neither $A_{ir}$ nor $A_{jr}$ happens,
then 
\begin{align*}
\left| {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right|=0.
\end{align*}
So we have
\begin{align*}
 \E_{\wt{w}_r}[s_r]\leq \E_{\wt{w}_r} \left[ \sum_{i=1}^n \sum_{j=1}^n{\bf 1}_{A_{ir}\cup A_{jr}} \right]\leq \frac {4n^2R}{\sqrt{2\pi}}   \leq 2n^2 R
\end{align*}
and
\begin{align*}
    \E_{\wt{w}_r} \left[ \left(s_r-\E_{\wt{w}_r}[s_r] \right)^2 \right]\leq \E_{\wt{w}_r}[s_r^2]\leq \E_{\wt{w}_r} \left[ \left(\sum_{i=1}^n \sum_{j=1}^n{\bf 1}_{A_{ir}\cup A_{jr}} \right)^2 \right]
     \leq \frac {8n^4R}{\sqrt{2\pi}}  
     \leq 4 n^4 R
\end{align*}
We also have $|s_r|\leq n^2$.
So we can apply Bernstein inequality to get for all $t>0$,
\begin{align*}
    \Pr \left[\sum_{r=1}^m s_r\geq 2mn^2R +mt \right]
    &\leq \Pr \left[\sum_{r=1}^m (s_r-\E[s_r])\geq mt \right]\\
    &\leq \exp \left( - \frac{ m^2t^2/2 }{ 4mn^4 R   + mn^2t/3 } \right).
\end{align*}
Choosing $t = n^2 R$, we get
\begin{align*}
    \Pr \left[\sum_{r=1}^m s_r\geq 3mn^2R  \right]
    \leq \exp \left( -\frac{ m^2 n^4 R^2 /2 }{ 4 m n^4 R + m n^4 R /3 } \right) \leq \exp \left( -\frac{m R}{10} \right)
\end{align*}
\end{proof}


\begin{lemma}[perturb both $w$ and $x$, general version of Lemma 3.2 in \cite{dzps19}]
Let $R = \frac{ c \delta \lambda_0 }{ n^2 }$, let $\beta = \frac{3 R}{ \sqrt{ 2d + \log (1/R) } }$. 
If $\wt{w}_1, \cdots, \wt{w}_m$ are i.i.d. generated from $\N(0,1)$, then with probability at least $1-\delta$, the following holds. 
For any set of weight vectors $w_1, \cdots, w_m \in \R^d$ that satisfy for any $r \in [m]$, $\| \wt{w}_r - w_r \|_2 \leq R$. For any set of vectors $x_1, \cdots, x_n$ and $\wt{x}_1, \cdots, \wt{x}_n$ that satisfy, $\| x_i - \wt{x}_i \|_2 \leq \beta, \forall i \in [n]$.  Let $H \in \R^{n \times n}$ be defined, 
\begin{align*}
H_{i,j} (x, w) = & ~ \frac{1}{m} x_i^\top x_j \sum_{ r = 1 }^m \mathds{1}_{ w_r^\top x_i \geq 0, w_r^\top x_j \geq 0 } \\
\wt{H}_{i,j} (  \wt{x}, \wt{w} ) = & ~ \frac{1}{m} \wt{x}_i^\top \wt{x}_j \sum_{ r = 1 }^m \mathds{1}_{ \wt{w}_r^\top \wt{x}_i \geq 0, \wt{w}_r^\top \wt{x}_j \geq 0 }
\end{align*}
Then we have
\begin{align*}
 \| H(x,w) - H(\wt{x},\wt{w}) \|_2< \frac{1}{4} \lambda_0 \text{~~~and~~~} \lambda_{\min} (H) > \frac{1}{2} \lambda_0
\end{align*}
\end{lemma}

\begin{proof}
We define event $A_{i,r}$ as follows:
\begin{align*}
A_{i,r} = \left\{ \exists u : \| u - \wt{w}_r \|_2 \leq R, \| x_i - \wt{x}_i \|_2 \leq \beta ,  {\bf 1}_{ \wt{x}_i^\top \wt{w}_r \geq 0 } \neq {\bf 1}_{ x_i^\top u \geq 0 } \right\}.
\end{align*}
Then we claim that if $A_{i,r}$ happens,
then we must have $|\wt{w}_r^\top \wt{x}_i|\leq \beta\|\wt{w}_r\|_2+R$.
This is because for all $u$ such that $ \| u - \wt{w}_r \|_2 \leq R$,
\begin{align*}
    |\wt{w}_r^\top \wt{x}_i-u^\top x_i|
    = & ~ |\wt{w}_r^\top \wt{x}_i-\wt{w}_r^\top x_i+\wt{w}_r^\top x_i-u^\top x_i| \\
    \leq & ~ |\wt{w}_r^\top \wt{x}_i-\wt{w}_r^\top x_i|+|\wt{w}_r^\top x_i-u^\top x_i|\\
    \leq & ~ \beta\cdot \|\wt{w}_r\|_2+R
\end{align*}
Hence when $|\wt{w}_r^\top \wt{x}_i|> \beta\|\wt{w}_r\|_2+R$,
$\wt{w}_r^\top \wt{x}_i$ and $u^\top x_i$ have the same sign.
%\textcolor{red}{If we can show for proper setting of $\beta$, $\Pr[|\wt{w}_r^\top \wt{x}_i|\leq  \beta\|\wt{w}_r\|_2+R]=O(R)$, then the same argument still works.}

Since Gaussian distribution is invariant under rotation,
without losing generality we may assume $\tilde x_i=(\|\tilde x_i\|_2,0,0,\cdots,0)$.
Hence
\begin{align*}
    \Pr[|\wt{w}_r^\top \wt{x}_i|\leq  \beta\|\wt{w}_r\|_2+R]
    =&\int_{0}^{\infty} \Pr\left[|\wt{w}_r^\top \wt{x}_i| \leq  \beta\|\wt{w}_r\|_2+R ~\Big|~     |(\wt{w}_r)_1|=t\right] \cdot \Pr\left[|(\wt{w}_r)_1|=t\right] \d t\\
    =&\int_{0}^{\infty} \Pr\left[\left( \sum_{j=2}^d (\wt{w}_r)_j^2 \right)^{1/2} \geq \left(\frac{t\|\wt{x}_i\|_2-R} {\beta} \right)\right] \cdot \Pr\left[|(\wt{w}_r)_1|=t\right] \d t\\
\end{align*}

We have
\begin{align*}
    d-1+2\sqrt{(d-1)\log (1/ R)}+2\log (1/ R)
    \leq & ~ 2d+3\log ( 1 / R )  \\
    = & ~ \left(\frac{3R} {\beta} \right)^2 & \text{~by~choice~of~} \beta \\
    \leq & ~ \left(\frac{4R\cdot(1-\beta)-R} {\beta} \right)^2 \\
    \leq & ~ \left(\frac{t\|\wt{x}_i\|_2-R} {\beta} \right)^2 & \text{~by~} t\geq 4R
\end{align*}
By Lemma \ref{lem:chi_square_tail},
when $t\geq 4R$,
\begin{align*}
   \Pr\left[\left( \sum_{j=2}^d (\wt{w}_r)_j^2 \right)^{1/2} \geq \left(\frac{t\|\wt{x}_i\|_2-R} {\beta} \right)\right]&\leq  \Pr\left[\sum_{j=2}^d (\wt{w}_r)_j^2\geq \left(\frac{t\|\wt{x}_i\|_2-R} {\beta} \right)^2\right]\\
&\leq \Pr \left[\sum_{j=2}^d (\wt{w}_r)_j^2\geq d-1+2\sqrt{(d-1)\log \frac 1 R}+2\log \frac 1 R \right]\\
&\leq e^{-\log \frac 1 R}=R
\end{align*}
Therefore
\begin{align*}
    &\int_{0}^{\infty} \Pr\left[\left( \sum_{j=2}^d (\wt{w}_r)_j^2 \right)^{1/2} \geq \left(\frac{t\|\wt{x}_i\|_2-R} {\beta} \right)\right] \cdot \Pr\left[|(\wt{w}_r)_1|=t\right] \d t\\
    \leq & \int_{0}^{4R}  \Pr\left[|(\wt{w}_r)_1|=t\right] \d t
    + \int_{4R}^{+\infty} \Pr\left[\left( \sum_{j=2}^d (\wt{w}_r)_j^2 \right)^{1/2} \geq \left(\frac{t\|\wt{x}_i\|_2-R} {\beta} \right)\right] \cdot \Pr\left[|(\wt{w}_r)_1|=t\right] \d t\\
    \leq & \Pr[|(\wt{w}_r)_1|\leq 4R]+R\int_{4R}^{+\infty}  \Pr\left[|(\wt{w}_r)_1|=t\right] \d t\\
    \leq & \Pr[|(\wt{w}_r)_1|\leq 4R]+R\leq (\frac 8 {\sqrt{2\pi}}+1)R
\end{align*}
This gives us $\Pr[A_{ir}] \leq (\frac 8 {\sqrt{2\pi}}+1)R$.




\end{proof}

\begin{lemma}[perturb both $w$ and $x$, high probability, general version of Lemma 3.2 in \cite{dzps19}]
\Zhao{TODO}
Let $R = \frac{ c \delta \lambda_0 }{ n^2 }$, let $\beta = \frac{3 R}{ \sqrt{ 2d + \log (1/R) } }$. 
If $\wt{w}_1, \cdots, \wt{w}_m$ are i.i.d. generated from $\N(0,1)$, then with probability at least $1-\delta$, the following holds. 
For any set of weight vectors $w_1, \cdots, w_m \in \R^d$ that satisfy for any $r \in [m]$, $\| \wt{w}_r - w_r \|_2 \leq R$. For any set of vectors $x_1, \cdots, x_n$ and $\wt{x}_1, \cdots, \wt{x}_n$ that satisfy, $\| x_i - \wt{x}_i \|_2 \leq \beta, \forall i \in [n]$.  Let $H \in \R^{n \times n}$ be defined, 
\begin{align*}
H_{i,j} (x, w) = & ~ \frac{1}{m} x_i^\top x_j \sum_{ r = 1 }^m \mathds{1}_{ w_r^\top x_i \geq 0, w_r^\top x_j \geq 0 } \\
\wt{H}_{i,j} (  \wt{x}, \wt{w} ) = & ~ \frac{1}{m} \wt{x}_i^\top \wt{x}_j \sum_{ r = 1 }^m \mathds{1}_{ \wt{w}_r^\top \wt{x}_i \geq 0, \wt{w}_r^\top \wt{x}_j \geq 0 }
\end{align*}
Then we have
\begin{align*}
 \| H(x,w) - H(\wt{x},\wt{w}) \|_2< \frac{1}{4} \lambda_0 \text{~~~and~~~} \lambda_{\min} (H) > \frac{1}{2} \lambda_0
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
\sum_{i} \sum_j | \wt{H}_{i,j} - H_{i,j} | 
= & ~ \frac{1}{m} \sum_{i=1}^n \sum_{j=1}^n \left| x_i^\top x_j \sum_{r=1}^m ( {\bf 1}_{ \wt{w}_r^\top \wt{x}_i \geq 0, \wt{w}_r^\top \wt{x}_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } ) \right|  \\
\leq & ~ \frac{1}{m} \sum_{i=1}^n \sum_{j=1}^n \sum_{r=1}^m \left| {\bf 1}_{ \wt{w}_r^\top \wt{x}_i \geq 0, \wt{w}_r^\top \wt{x}_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right| \\
= & ~ \frac{1}{m} \sum_{r=1}^m  \sum_{i=1}^n \sum_{j=1}^n \left| {\bf 1}_{ \wt{w}_r^\top \wt{x}_i \geq 0, \wt{w}_r^\top \wt{x}_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right|
\end{align*}


Define $s_r=\sum_{i=1}^n \sum_{j=1}^n\left| {\bf 1}_{ \wt{w}_r^\top \wt{x}_i \geq 0, \wt{w}_r^\top \wt{x}_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right|$.
Then $s_r$ is a random variable that only depends on $\wt{w}_r$.
Since $\{\wt{w}_r\}_{r=1}^m$ are independent,
$\{s_r\}_{r=1}^m$ are also mutually independent.

If neither $A_{ir}$ nor $A_{jr}$ happens,
then 
\begin{align*}
\left| {\bf 1}_{ \wt{w}_r^\top \wt{x}_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } \right|=0.
\end{align*}
So we have
\begin{align*}
 \E_{\wt{w}_r}[s_r]\leq \E_{\wt{w}_r} \left[ \sum_{i=1}^n \sum_{j=1}^n{\bf 1}_{A_{ir}\cup A_{jr}} \right]\leq {2(\frac 8 {\sqrt{2\pi}}+1)n^2R} \leq 9n^2R
\end{align*}
and
\begin{align*}
    \E_{\wt{w}_r} \left[ \left(s_r-\E_{\wt{w}_r}[s_r] \right)^2 \right]\leq \E_{\wt{w}_r}[s_r^2]\leq \E_{\wt{w}_r} \left[ \left(\sum_{i=1}^n \sum_{j=1}^n{\bf 1}_{A_{ir}\cup A_{jr}} \right)^2 \right]
     \leq 4(\frac 8 {\sqrt{2\pi}}+1)n^4R \leq 17n^4R
\end{align*}
We also have $|s_r|\leq n^2$.
So we can apply Bernstein inequality to get for all $t>0$,
\begin{align*}
    \Pr \left[\sum_{r=1}^m s_r\geq 9mn^2R +mt \right]
    &\leq \Pr \left[\sum_{r=1}^m (s_r-\E[s_r])\geq mt \right]\\
    &\leq \exp \left( - \frac{ m^2t^2/2 }{ 17mn^4 R   + mn^2t/3 } \right).
\end{align*}
Choosing $t = n^2 R$, we get
\begin{align*}
    \Pr \left[\sum_{r=1}^m s_r\geq 10mn^2R  \right]
    \leq \exp \left( -\frac{ m^2 n^4 R^2 /2 }{ 17 m n^4 R + m n^4 R /3 } \right) \leq \exp \left( -\frac{m R}{36} \right)
\end{align*}
\end{proof}

Fix $y\in \R^n$ so that $\|y\|=1$.
Let $z=(\wt{H}-H)y$.
Then
\[
z_i=\frac 1 m\sum_{j=1}^n y_j\cdot x_i^\top x_j \sum_{r=1}^m ( {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_j \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_j \geq 0 } ),
\]
and
\[
|z_i|\leq \sqrt{n} 
\]
Hence
\begin{align*}
 \E[z_i^2]=&\E[\frac 1 {m^2} \sum_{j_1,j_2} y_{j_1}y_{j_2}\cdot x_i^\top x_{j_1}\cdot x_i^\top x_{j_2}
\left(\sum_{r=1}^m ( {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_{j_1} \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_{j_1} \geq 0 } )\right)\\
&\left(\sum_{r=1}^m ( {\bf 1}_{ \wt{w}_r^\top x_i \geq 0, \wt{w}_r^\top x_{j_2} \geq 0} - {\bf 1}_{ w_r^\top x_i \geq 0 , w_r^\top x_{j_2} \geq 0 } )\right)]\\ 
&\leq \E[\frac 1 {m^2} \sum_{j_1,j_2} y_{j_1}y_{j_2}\cdot x_i^\top x_{j_1}\cdot x_i^\top x_{j_2}
\left(\sum_{r=1}^m {\bf 1}_{A_{ir}\cup A_{j_1r}} \right)\left(\sum_{r=1}^m {\bf 1}_{A_{ir}\cup A_{j_2r}} \right)] ?\\
&=\frac 1 {m^2} \sum_{j_1,j_2} y_{j_1}y_{j_2}\cdot x_i^\top x_{j_1}\cdot x_i^\top x_{j_2}\E[
\left(\sum_{r=1}^m {\bf 1}_{A_{ir}\cup A_{j_1r}} \right)\left(\sum_{r=1}^m {\bf 1}_{A_{ir}\cup A_{j_2r}} \right)]\\
&\leq \frac 1 {m^2} \sum_{j_1,j_2} y_{j_1}y_{j_2}\cdot x_i^\top x_{j_1}\cdot x_i^\top x_{j_2}(m\cdot 13R+m(m-1)\cdot 17R)\\
&\leq 17R\cdot \|y\|_1^2\leq 17Rn
\end{align*}



\begin{comment}
\Zhao{What is erfc? Even if $R$ is super small, it doesn't work?} 

Can we do this instead?
\begin{align*}
&  \int_{0}^{\infty} \Pr\left[\sum_{j=2}^d (\wt{w}_r)_j^2\geq \left(\frac{t\|\wt{x}_i\|_2-R} {\beta} \right)^2\right] \cdot \Pr\left[|(\wt{w}_r)_1|=t\right] \d t\\
    \leq &    \int_{0}^{2R}  \Pr\left[|(\wt{w}_r)_1|=t\right] \d t
    + \sum_{i=1}^{\infty} \int_{2^i R}^{ 2^{i+1} R} e^{-t^2}\cdot \left( \frac 2 {\sqrt{2\pi}}e^{-\frac {t^2} 2} \right)\d t\\
\end{align*}

\end{comment}

\begin{comment}

\Zhao{Trash calculations start from here}
Given $|| x_i - x_i(0) ||_2 < c_1$

\begin{align*}
  & ~  x_i x_j \sum \mathds{1}_{ w x_i, w x_j } - x_i(0) x_j(0) \sum \mathds{1}_{ w (0) x_i(0), w(0) x_j(0) } \\
= & ~  x_i x_j \sum \mathds{1}_{ w x_i, w x_j } - x_i x_j \sum \mathds{1}_{ w(0) x_i, w(0) x_j } \\ 
+ & ~ x_i x_j \sum \mathds{1}_{ w(0) x_i, w(0) x_j } - x_i(0) x_j(0) \sum \mathds{1}_{ w(0) x_i, w(0) x_j } \\
+ & ~ x_i(0) x_j(0) \sum \mathds{1}_{ w(0) x_i, w(0) x_j } - x_i(0) x_j(0) \sum \mathds{1}_{ w(0) x_i(0), w(0) x_j(0) } 
\end{align*}

\begin{align*}
 E_{w} [ |  \mathds{1}_{ w x } - \mathds{1}_{w x(0)} | ] \approx \| x - x(0) \|_2
\end{align*}

\begin{align*}
 E_{w} [ |  \mathds{1}_{ w x(0) + w delta_x } - \mathds{1}_{w x(0)} | ] \approx \| x - x(0) \|_2
\end{align*}
\end{comment}

==> trash.tex <==
\begin{comment}

\subsection{Discussion, Simon and Zhao}

We consider the following optimization problem
\begin{align*}
    \min_w \max_{ x \in B_r(x^*) } ( f(w,x) - y )^2
\end{align*}

\subsubsection{Case $d=1$, $n=1$, $\phi(x) = x$, the data is $(0,0)$.}

For a single data $(x,y)$, we define the Loss function as follows:
\begin{align*}
    L = \frac{1}{2} ( f(w,x) - y )^2 .
\end{align*}

We compute the gradient of $L$ with respect to $x$,
\begin{align*}
 \frac{ \partial L}{ \partial x } = ( y - w^\top x) w.
\end{align*}
Then, we have consider the following quantity,
\begin{align*}
    \langle \frac{ \partial L}{ \partial x } , x \rangle = ( y - w^\top x) w^\top x
\end{align*}
where
\begin{align*}
f(x) = w^\top \phi(x) = w^\top x.
\end{align*}

There exists $w \in \R$ such that
\begin{align*}
| ( w^\top x - y ) w | \leq \epsilon < \gamma .
\end{align*}
We consider a special case where $x^* = 0$ and $y^* = 0$. The feasible range of $x$ is $[-\gamma, +\gamma]$.
\begin{align*}
    | (w^\top x - y) w |= | w^2 x | \leq \epsilon.
\end{align*}
We know that $|x| \leq \gamma$. Therefore, as long as we choose small enough $w \in \R$.

\subsubsection{Case $d=1$, $n=1$, $\phi(x)$, the data is $(x_0,y_0)$}

For a single data $(x,y)$, we define the Loss function as follows:
\begin{align*}
    L = \frac{1}{2} ( f(w,x) - y )^2 .
\end{align*}

We compute the gradient of $L$ with respect to $x$,
\begin{align*}
 \frac{ \partial L}{ \partial x } = ( y - w^\top x) w.
\end{align*}
Then, we have consider the following quantity,
\begin{align*}
    \langle \frac{ \partial L}{ \partial x } , x \rangle = ( y - w^\top x) w^\top x
\end{align*}
where
\begin{align*}
f(x) = w^\top \phi(x) = w^\top x.
\end{align*}

There exists $w \in \R$ such that
\begin{align*}
| ( w^\top x - y ) w | \leq \epsilon < \gamma .
\end{align*}

The feasible range of $x$ is $[x_0 - \gamma, x_0 + \gamma]$.
\begin{align*}
| (w x - y) w | \leq \epsilon
\end{align*}

\begin{enumerate}
    \item $( w x - y ) w \geq 0$
    \begin{enumerate}
        \item $(wx - y) \geq 0$ and $w \geq 0$. \\
        It becomes $(wx - y) w \leq \epsilon$, which is equivalent to $x\cdot w^2 - y \cdot w - \epsilon \leq 0$. Thus it requires
        \begin{align*}
           \frac{y - \sqrt{y^2 + 4 x \epsilon} }{2x} \leq  w \leq \frac{y + \sqrt{y^2 + 4 x \epsilon} }{2x}
        \end{align*}
        \begin{enumerate}
            \item If $x_0 - \gamma > 0$, then $wx - y \geq 0$ implies $w \geq \frac{y}{x}$. Thus the feasible region for $w$ should be 
            \begin{align*}
            \left[ \frac{y}{x} , \frac{ y + \sqrt{y^2 + 4 x \epsilon} }{2x} \right]
            \end{align*}
            \item Otherwise
        \end{enumerate}
        \item $(wx - y) \leq 0$ and $w \leq 0$ 
    \end{enumerate}
    \item $( w x - y ) w \leq 0$
    \begin{enumerate}
        \item $(wx - y) \geq 0$ and $w \leq 0$
        \item $(wx - y) \leq 0$ and $w \geq 0$
    \end{enumerate}
\end{enumerate}

\end{comment}

\begin{comment}
We compute the difference between two terms
\begin{align*}
& ~ \wt{x}_i^\top \wt{x}_j \mathds{1}_{ w^\top \wt{x}_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } - x_i^\top x_j \mathds{1}_{ w^\top x_i \geq 0} \mathds{1}_{ w^\top x_j \geq 0 }  \\
= & ~ \wt{x}_i^\top \wt{x}_j \mathds{1}_{ w^\top \wt{x}_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } - x_i^\top \wt{x}_j \mathds{1}_{ w^\top \wt{x}_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } \\
+ & ~ x_i^\top \wt{x}_j \mathds{1}_{ w^\top \wt{x}_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } - x_i^\top x_j \mathds{1}_{ w^\top \wt{x}_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } \\
+ & ~ x_i^\top x_j \mathds{1}_{ w^\top \wt{x}_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } - x_i^\top x_j \mathds{1}_{ w^\top x_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } \\
+ & ~ x_i^\top x_j \mathds{1}_{ w^\top x_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } - x_i^\top x_j \mathds{1}_{ w^\top x_i \geq 0} \mathds{1}_{ w^\top x_j \geq 0 } \\
= & ~ \delta_{x,i}^\top \wt{x}_j \mathds{1}_{w^\top \wt{x}_i \geq 0} \mathds{1}_{ w^\top \wt{x}_j \geq 0 } + x_i^\top \delta_{x,j} \mathds{1}_{w^\top \wt{x}_i \geq 0} \mathds{1}_{w^\top \wt{x}_j \geq 0} \\
+ & ~ x_i^\top x_j g_i' \mathds{1}_{w^\top \wt{x}_j \geq 0} + x_i^\top x_j \mathds{1}_{ w^\top \wt{x}_i } g_j'
\end{align*}   
where $g_i' = \mathds{1}_{w^\top \wt{x}_i \geq 0} - \mathds{1}_{w^\top x_i \geq 0}$

One trivial fact is $\mathds{1}_{ x >= 0 } - \mathds{1}_{ y >= 0 }$ is not always equal to $\mathds{1}_{ x - y >= 0 }$.
\end{comment}


\subsection{Following the technique of Finding Nash}
We can follow the framework defined in \cite{h16}.

In page 146 of textbook by Elad \cite{h16}, it proved Eq. (8.1). We need that equation for neural network function $f$.

---
Then, by appropriate choice of $\eta$ and Corollary 5.5, we have
\begin{align*}
\sum_t f_t ( x_t ) \leq \min_{ x^* \in K } \sum_t f_t ( x^* ) + \sqrt{2 T \log n}.
\end{align*}
---

We have function $f(w, x, y)$, suppose we have $n$ datas $\{ (x_1,y_1) , (x_2,y_2) , \cdots , (x_n, y_n) \}$:
\begin{align*}
a
\end{align*}

Also, page 265 in Bubeck book.

\subsection{Using Allen-Zhu et al.'s paper}



\section{Gradient Attack}
We define function $f : \R^{d \times m} \times \R^{d \times m} \times \R^d \rightarrow \R$
\begin{align*}
    f(W,\tilde{W},x) = \frac{1}{\sqrt{m}}\sum_{r=1}^m a_r \inner{w_r}{x}\ind_{ \inner{\tilde{w}_r}{x} \geq 0}
\end{align*}

Two-layer ReLU network:
\begin{align*}
    f(W,W,x) = \frac{1}{\sqrt{m}}\sum_{r=1}^m a_r \inner{w_r}{x}\ind_{ \inner{w_r}{x} \geq 0}
\end{align*}
Pseudo version of Two-layer ReLU network: 
\begin{align*}
    f(W, W^{(0)}, x) = \frac{1}{\sqrt{m}}\sum_{r=1}^m a_r \inner{w_r}{x} \ind_{ \langle w_r^{(0)}, x \rangle \geq 0}
\end{align*}
Let $\hat{x} := A(W, x)$ be the adversarial example of net $f_W$ acting on a normal example $x$. Similarly $\hat{S} := A(W, S)$ is the dataset generated by $A$ acting on each $x\in S$.\\

Definitions of regularized loss and regularized pseudo-loss
\begin{align*}
    l(W, S) := & ~ \frac{1}{|S|}\sum_{(x,y)\in S} \loss(f(W,W,x), y) + \alpha \cdot \|W - W^{(0)}\|_F^2\\
    \tilde{l}(W, S) := & ~ \frac{1}{|S|}\sum_{(x,y)\in S} \loss(f(W,W^{(0)},x), y) + \alpha \cdot \|W - W^{(0)}\|_F^2
\end{align*}
We define
\begin{align*}
    \nabla_{r}^{(t)} := & ~ \nabla_{w_r} l(W^{(t)}, S^{(t)}) & \in \R^d, \\
    \tilde{\nabla}_{r}^{(t)} := & ~ \nabla_{w_r} \tilde{l}(W^{(t)}, S^{(t)}) & \in \R^d.
\end{align*}

\begin{theorem}[Lipschitzness of $A$ w.r.t $W$]
\begin{align*}
    \|A(W, x) - A(W', x)\|_2 \leq L_A \cdot \|W - W'\|_F
\end{align*}
\end{theorem}
\begin{proof}
{\color{red}TODO.}
\end{proof}

\subsection{Convergence}

Recall that the definition of $\| \cdot \|_{2,\infty}$-norm and $\| \cdot \|_{2,1}$. For a matrix $W \in \R^{d\times m}$, $\| W \|_{2,\infty} = \max_{r \in [m]} \| W_r \|_2$ where $W_r$ is the $r$-th column of matrix $W$, for all $r \in [m]$. For a matrix $W \in \R^{d \times m}$, $\| W \|_{2,1} = \sum_{r=1}^m \| W_r \|_2$.
\begin{lemma} 
\label{lemma:coupling}
For any iteration $t$, if $\| W^{(t)} - W^{(0)}\|_{2,\infty}\leq \frac{1}{\sqrt{m}}$, then we have
\begin{align*}
  \| \tilde{\nabla}^{(t)} - \nabla^{(t)} \|_{2,1} = O(1)
\end{align*}
\begin{proof}
Assuming for all $r\in[m], \| w_r^{(t)} - w_r^{(0)}\|_2  = O(\frac{1}{\sqrt{m}})$, we know for $\Omega(m - \sqrt{m})$ nodes $r\in[m]$ such that 
$\| \tilde{\nabla}_r^{(t)} - \nabla_{r}^{(t)} \|_2 = 0$ 
and for the rest $O(\sqrt{m})$ nodes
\begin{align*}
\| \tilde{\nabla}_{r}^{(t)} - \nabla_{r}^{(t)} \|_2 \leq \frac{|a_r|}{\sqrt{m}} \frac{1}{n} \sum_{i=1}^n \left|\ind_{\inner{w_r^{(t)}}{x_i} \geq 0 } - \ind_{\inner{w_r^{(0)}}{x_i}\geq 0 }\right| \|x_i\|_2 \leq \frac{1}{\sqrt{m}}
\end{align*}
Thus we conclude
\begin{align*}
    \sum_{r=1}^m \| \tilde{\nabla}_{r}^{(t)} - \nabla_{r}^{(t)} \|_2 \leq \sqrt{m} \frac{1}{\sqrt{m}} = 1
\end{align*}
\end{proof}
\end{lemma}

Following the gradient step, 

\Zhao{What is $W^*$, it is never defined anywhere.}

By the strong convexity of $\tilde{l}$ w.r.t $W$, 
\begin{align}\label{eq:bound_diff_W_t_and_W_star}
    \tilde{l}(W^{(t)}, S^{(t)}) - \tilde{l}(W^*, S^{(t)}) &\leq \inner{\tilde{\nabla}^{(t)}}{W^{(t)} - W^*} - \alpha \| W^{(t)} - W^* \|_F^2 \notag\\
    &= \inner{\nabla^{(t)}}{W^{(t)} - W^*} - \alpha \| W^{(t)} - W^* \|_F^2 + \inner{\tilde{\nabla}^{(t)} - \nabla^{(t)}}{W^{(t)} - W^*} \notag \\
    &\leq \inner{\nabla^{(t)}}{W^{(t)} - W^*} - \alpha \| W^{(t)} - W^* \|_F^2 + O(\frac{1}{\sqrt{m}})
\end{align}
where the last step is due to the lemma~\ref{lemma:coupling} as follows
\begin{align*}
\inner{\tilde{\nabla}^{(t)} - \nabla^{(t)}}{W^{(t)} - W^*} \leq \| \tilde{\nabla}^{(t)} - \nabla^{(t)} \|_{2,1} \cdot \|W^{(t)} - W^*\|_{2,\infty} = O(\frac{1}{\sqrt{m}}).
\end{align*}

Next goal is to upper bound the first term in Eq.~\eqref{eq:bound_diff_W_t_and_W_star}. For each $r\in[m]$, 
\begin{align*}
    \inner{\nabla_{r}^{(t)}}{w_r^{(t)} - w_r^*} &\leq \frac{1}{2 \eta_t} ( \| w_r^t - w_r^* \|_2^2 - \| w_r^{t+1} - w_r^* \|_2^2 ) + \frac{\eta_t}{2} \| \nabla_{r}^{(t)} \|_2^2 - \alpha \| w_r^{(t)} - w_r^* \|_2^2
\end{align*}
Taking the summation over all $r \in [m]$, we have
\begin{align*}
    \inner{\nabla^{(t)}}{W^{(t)} - W^*} \leq \frac{1}{2 \eta_t} ( \| W^t - W^* \|_F^2 - \| W^{t+1} - W^* \|_F^2 ) + \frac{\eta_t}{2} \| \nabla^{(t)} \|_F^2 - \alpha \| W^{(t)} - W^* \|_F^2
\end{align*}
Therefore, we have
\begin{align*}
    \sum_{t=1}^T  \tilde{l}(W^{(t)}, S^{(t)})  - \sum_{t=1}^T \tilde{l}(W^*, S^{(t)})
    \leq & ~ \sum_{t=1}^T \left( \inner{\nabla^{(t)}}{W^{(t)} - W^*} - \alpha \| W^{(t)} - W^* \|_F^2 + O(\frac{1}{\sqrt{m}}) \right) \\
    \leq & ~ \sum_{t=1}^T \|W^{(t)} - W^*\|_F^2(\frac{1}{\eta_t} - \frac{1}{\eta_{t-1}} - \alpha) + G^2\sum_{t=1}^T \eta_t +  O\left( \frac{T}{\sqrt{m}} \right) 
\end{align*}
\Zhao{I don't see how to reach the last step, and we never define $G$.}

If we choose $m=\Omega\left(\frac{1}{\varepsilon^3}\right)$, $T = \tilde{\Omega}\left(\frac{G^2}{\varepsilon^3}\right)$, $\alpha=O\left(\varepsilon\right)$, and $\eta_t=\frac{1}{2\alpha (t+1)}$, we can conclude
\begin{align*}
    \frac{1}{T}\sum_{t=1}^T  \tilde{l}(W^{(t)}, S^{(t)}) - \frac{1}{T} \sum_{t=1}^T \tilde{l}(W^*, S^{(t)}) &\leq \frac{G^2 \log T}{\alpha T} + O\left(\frac{1}{\sqrt{m}}\right) \leq \varepsilon
\end{align*}

Furthermore, $w_r^{(t)}$ converges to $w_r^*$ as well since
\begin{align*}
\|w_r^{(t+1)} - w_r^*\|_2^2 &\leq  (1 - 2\alpha \eta_t)\|w_r^{(t)} - w_r^*\|_2^2 + \eta_t^2 G_r^2 + \eta_t\left( \tilde{l}(W^*, S^{(t)}) - \tilde{l}(W^{(t)}, S^{(t)})\right) \\
&\leq \| w_r^{(0)} - w_r^*\|_2^2 \prod_{\tau=1}^t (1 - 2\alpha \eta_\tau)  + \frac{1}{m}\sum_{\tau=1}^{t}\eta_\tau^2 \prod_{s=\tau+1}^{t} (1 - 2\alpha \eta_{s-1}) \\
&\leq \frac{ \| w_r^{(0)} - w_r^*\|_2^2}{t+1} + \frac{\log t}{m\varepsilon^2 t} \\
& = \tilde{O}\left(\frac{1}{m\varepsilon^2 t}\right)
\end{align*}
where the last step follows from \Zhao{???}.

And also, $w_r^{(t)}$ stays in a small neighborhood around $w_r^{(0)}$ for all $t\in[T]$ and $r\in[m]$ because
\begin{align*}
    \| w_r^{(t)} - w_r^{(0)}\|_2 \leq G_r\sum_{\tau=1}^T \eta_\tau \leq \frac{\log T}{\alpha\sqrt{m}} = \tilde{O}\left(\frac{1}{\epsilon\sqrt{m}}\right)
\end{align*}

